ArtiSG: Functional 3D Scene Graph Construction via Human-demonstrated Articulated Objects Manipulation

3D scene graphs have empowered robots with semantic understanding for navigation and planning. However, current functional scene graphs primarily focus on static element detection, lacking the actionable kinematic information required for physical manipulation, particularly regarding articulated objects. Existing approaches for inferring articulation mechanisms from static observations are prone to visual ambiguity, while methods that estimate parameters from state changes typically rely on constrained settings such as fixed cameras and unobstructed views. Furthermore, inconspicuous functional elements like hidden handles are frequently missed by pure visual perception. To bridge this gap, we present ArtiSG, a framework that constructs functional 3D scene graphs by encoding human demonstrations into structured robotic memory. Our approach leverages a robust data collection pipeline utilizing a portable hardware setup to accurately track 6-DoF manipulation trajectories and estimate articulation axes, even under camera ego-motion. By integrating these kinematic priors into a hierarchical, open-vocabulary graph, our system not only models how articulated objects move but also utilizes physical interaction data to discover implicit elements. Extensive real-world experiments demonstrate that ArtiSG significantly outperforms baselines in functional element recall and articulation estimation precision. Moreover, we show that the constructed graph serves as a reliable robotic memory, effectively guiding robots to perform language-directed manipulation tasks in real-world environments containing diverse articulated objects.

==> general_response.tex <==
We thank the reviewers for their constructive feedback and valuable suggestions.  
All raised concerns have been carefully addressed through comprehensive revisions \textcolor{blue}{marked in blue} throughout the manuscript.  
The major changes are summarized as follows:

\begin{enumerate}
    \item \textbf{Clarified contribution framing:}  
    We have revised the abstract and \Cref{sec:intro} to clearly position our contribution.

    \item \textbf{Expanded baselines and restructured evaluations:}  
    We have added FunGraph, Fun3DU and ArtiPoint as our baselines. We have also revised \Cref{sec:exp} to ensure fairer and more informative comparisons across input modalities.

    \item \textbf{Improved experimental clarification and ablation studies:}  
    We have clarified multiple details, including fair manipulation sequences for comparison, articulation type selection, unified coordinate alignment, IoU threshold settings, and functionality prompt design. In addition, we have added ablation studies to validate the effectiveness of our top-$k$ selection strategy.

    \item \textbf{Clarified scene graph initialization module novelty:}  
    We have clarified that the scene graph initialization module is not the primary contribution of our work, but it differs from prior methods in both its workflow and advantages.   
    
    \item \textbf{Clarified hardware design choices:}  
    We explicitly state that the hardware-assisted tracking setup is a deliberate system-level design choice to guarantee high-fidelity kinematic priors. 
    %% 完成时态改成will
    The 3D-printable hardware models, assembly instructions, and tracking code to facilitate reproduction will soon be made publicly available.

\end{enumerate}

Below, we provide detailed point-by-point responses to each reviewer.

==> reviewer1.tex <==
\subsection{Regarding More Baselines}
We completely agree with the reviewer and appreciate the valuable suggestions. 
In our revised manuscript, we have added Fun3DU as a primary baseline in the functional scene graph evaluation (\Cref{sec:eval_graph}), and ArtiPoint in the articulation tracking evaluation (\Cref{sec: eval_tracking}).

\subsection{Regarding Tracking Hardware}
We acknowledge that relying on marker-based hardware limits immediate in-the-wild deployment. 
However, this design choice deliberately prioritizes the high-fidelity kinematic precision strictly required for reliable axis estimation and downstream robotic execution. 
We have also explicitly acknowledged this limitation in the conclusion section (\Cref{sec:con}) and identified improving hardware portability as an important direction for future work.

To mitigate the hardware barrier and facilitate easy reproduction by the community, 
% 改成will
the following material will soon be open-sourced: 
1) the 3D-printable models and assembly instructions for the hardware, 
and 2) the accompanying tracking algorithms.


\subsection{Regarding Tracking Comparison}
We thank the reviewer for raising this critical concern regarding fair comparison and apologize for the lack of clarity in our initial manuscript. 
To ensure absolute fairness, we actually collect two separate sets of manipulation sequences: 
one using our hardware setup, 
and one using only bare hands. 
All vision-only baselines are evaluated exclusively on the bare-hand sequences.
We have explicitly clarified this experimental setup in \Cref{sec: eval_tracking}.

==> reviewer2.tex <==
% \begin{table}[t!]
% \centering
% \color{blue} % 让当前表格环境内的所有文字变为蓝色
% \caption{Functionality Segmentation Evaluation on SceneFun3D}
% \setlength{\tabcolsep}{10pt} % <--- 在这里添加，数值可以根据你的喜好微调
% \begin{tabular}{ccc}
% \toprule
% \textbf{\makecell{Affordance \\ (arti. type)}} & FunGraph & \makecell{ArtiSG\\(w.o. human)} \\
% \midrule
% Rotate     & \bf{25.6} & 25.0 \\
% Pinch Pull & 24.8      & \bf{83.5} \\
% Hook Pull  & \bf{10.1} & 0.0 \\
% Hook Turn  & \bf{37.7} & 24.1 \\
% \midrule
% \textbf{Average} & 24.6 & \bf{33.15}\\
% \bottomrule
% \end{tabular}
% \label{table:affordance}
% \end{table}

\subsection{Regarding Static Functional Element Detection Novelty and Evaluation Dataset Selection}
We clarify that the scene graph initialization module is not the primary contribution of our paper, but rather a necessary foundational step to ensure basic semantic awareness before human interaction begins. 
Fun3DU targets task-driven 3D segmentation rather than scene graph construction.

Our scene graph initialization differs from prior works by adopting a ``3D Obj. $\rightarrow$ 2D Fun. Ele. $\rightarrow$ 3D Fun. Ele." projection strategy using lightweight detectors. 
%% shengyz: 增加说明，不需遍历所有frame，只需处理top-k frame
Instead of traversing all frames, the detection and segmentation process only needs to be applied to the selected top-$k$ frames with respect to each object node. 
This yields two main advantages:
\begin{enumerate}
    \item \textbf{High computational efficiency:}  As shown in our newly added runtime comparison \Cref{table:times}, our method processes scenes significantly faster.
    \item \textbf{Structural robustness:} By segmenting functional elements within the 2D bounding boxes of projected 3D objects and projecting back to the 3D object point cloud, the parent-child edges between objects and functional elements are naturally established, eliminating the complex and error-prone graph-edge association step required by other methods.
\end{enumerate}

%% 贴张表对比下处理速度
\begin{table}[t!]
\centering
% \color{blue} % 让当前表格环境内的所有文字变为蓝色
\caption{Time consumption evaluation}
\begin{tabular}{clc}
\toprule
\textbf{Scene} & \textbf{Method} & \textbf{Time(s)} \\

% 先Real
\midrule
\multirow{3}{*}{Real-world} 
& OpenFunGraph       & 1239.9 \\
& FunGraph           & 408.9  \\
& ArtiSG (ours)      & \bf{51.0} \\

% 后Sim
\midrule
\multirow{3}{*}{Simulation} 
& OpenFunGraph       & 316.1 \\
& FunGraph           & 157.3 \\
& ArtiSG (w.o human) & \bf{49.0} \\

\bottomrule
\end{tabular}
\label{table:times}
\end{table}

Regarding the dataset selection, we have revised our manuscript in \Cref{sec:eval_graph} to explicitly frame real-world environments as our primary evaluation focus, as they best validate our human-interaction pipeline. 
For simulation, we choose Behavior-1K over SceneFun3D because its environments are densely populated with articulated objects, perfectly aligning with our manipulation focus. 
Conversely, SceneFun3D targets static segmentation across broader, non-articulable affordances (e.g., light switches), making it incompatible with our full dynamic pipeline. 
To validate the robustness of our static initialization module on a standardized benchmark, we also evaluate it on SceneFun3D.

As shown in \Cref{table:scenefun3d}, on the 4 affordance types specifically relevant to articulation objects, our method achieves comparable average performance to FunGraph under the AP25 metric.

\begin{table}[t!]
\centering
% \color{blue} % 让当前表格环境内的所有文字变为蓝色
\caption{Functionality Segmentation Evaluation on SceneFun3D}
\begin{tabular}{lccccc}
\toprule
\textbf{Method (AP$_{25}$)} & Rotate & Pinch Pull & Hook Pull & Hook Turn & \textbf{Average} \\
\midrule
FunGraph & \bf{25.6} & 24.8 & \bf{10.1} & \bf{37.7} & 24.6 \\
ArtiSG (w.o human) & 25.0 & \bf{83.5} & 0.0 & 24.1 & \bf{33.15} \\
\bottomrule
\end{tabular}
\label{table:scenefun3d}
\end{table}

\subsection{Regarding Unfair and Incomplete Baselines in Table I}
The reviewer raises a highly valid point. 
Comparing methods with fundamentally different input modalities in the same table causes confusion. 
We have completely restructured this evaluation and rewritten \Cref{sec:eval_graph}. 
First, we remove Lost\&Found and replace it with the more appropriate FunGraph baseline. 
Second, we explicit state the input modalities for all methods in the text and table captions.
 
\subsection{Regarding More Baselines}
We completely agree with the reviewer.
We have integrated Fun3DU for functional element detection and ArtiPoint for articulation estimation into our experiments to provide a comprehensive comparison.

\subsection{Regarding Tracking Hardware and Methodological Novelty}
We completely agree with your insightful observation. 
Our mathematical formulation for axis estimation indeed relies on standard optimization techniques, and the strong quantitative results are fundamentally attributed to the high-quality trajectories provided by the hardware tracking. 

To address this transparently, we have revised the manuscript in \Cref{sec:intro} to explicitly clarify that our contribution lies strictly at the \textit{systems level}, rather than proposing a novel estimation algorithm. Our core innovation is designing a reliable, hardware-assisted pipeline capable of injecting high-precision, real-world kinematic priors into a structured 3D scene graph. 
We have also explicitly acknowledged this limitation in the conclusion section (\Cref{sec:con}) and identified improving hardware portability as an important direction for future work.

% 改成will 
To facilitate reproduction by the community, we will soon open-source the 3D-printable hardware models, assembly instructions, and the accompanying tracking code. 


\subsection{Regarding Downstream Robot Manipulation}
The primary objective of this experiment is to demonstrate that the manipulation trajectories encoded in our scene graph are sufficiently precise to be directly executed by a robot. 
To avoid overstating the scope of this experiment, we have revised \Cref{sec:application} by removing the comparison with VLM-based methods and instead emphasizing how ArtiSG helps resolve visual ambiguities that static perception alone cannot reliably capture.

We agree with the reviewer that robustness to object displacement is an important practical consideration. 
Although the stored trajectories are represented in the global scene frame during demonstration, the articulated object's pose and its associated kinematic trajectory remain geometrically consistent. Therefore, if the object is displaced, the robot can first estimate the updated object pose and then recover a new executable manipulation trajectory through the relative transformation between the object pose and the recorded articulation trajectory.
We appreciate this forward-looking suggestion and have added it to our discussion of future work, where integrating explicit pose adaptation with downstream manipulation policies will be an important next step.


\subsection{Regarding Functionality Classes}
In our framework, the predefined prompts are not restricted to a fixed, limited vocabulary and can be dynamically expanded based on task requirements. 
In our experiments, prompting with ``handle,'' ``knob,'' and ``button'' proves sufficient to cover the relevant functional elements. 
We have added this detail in \Cref{sec:eval_graph}.

\subsection{Regarding Open-vocabulary Features}
To demonstrate the functional element-level discrimination capability of our extracted open-vocabulary features, we utilized these features to match functional elements to fine-grained affordance labels in our new SceneFun3D evaluation. 
%shengyz: 加 As shown，说comparable不说strong
As shown in \Cref{table:scenefun3d}, the comparable performance on this benchmark directly validates that our features meaningfully distinguish between different functional elements.

\subsection{Regarding Unified Coordinate System}
To guarantee that the RGB-D mapping sequence and the dynamic manipulation sequences are perfectly aligned within a unified coordinate system, our system scans a large, fixed ArUco marker placed in the environment at the beginning of data collection. 
This establishes a globally consistent anchor frame. 
We have added this critical detail in \Cref{sec: refine}.

\subsection{Regarding Articulation Type Selection}
We apologize for the vagueness in the original manuscript. 
The articulation type is selected by comparing the reconstruction residuals of the prismatic and revolute models, utilizing the Bayesian Information Criterion (BIC) as the penalty term for model complexity. 
We have explicitly stated this criterion in \Cref{sec:tracking}.

\subsection{Regarding Experiment Details in \Cref{sec:eval_graph}}
Following the evaluation protocol established by OpenFunGraph, we utilize an IoU threshold of $> 0$ to ensure a fair comparison across methods. 
This threshold has now been explicitly specified in \Cref{sec:eval_graph}.

==> reviewer4.tex <==
\subsection{Regarding Contribution Framing}
We appreciate the reviewer for pointing out this important framing issue. 
We agree that our core contribution is not the introduction of functional 3D scene graphs themselves, but the extension of existing functional scene graph representations with articulation-aware kinematic information. 
Accordingly, we have revised both the abstract and \Cref{sec:intro} to clarify this distinction from the outset. 



\subsection{Regarding Static Functional Element Detection Novelty and Ablation Study}
We clarify that the scene graph initialization module is not the primary contribution of our paper, but rather a necessary foundational step to ensure basic semantic awareness before human interaction begins. 
Our scene graph initialization differs from prior works by adopting a ``3D Obj. $\rightarrow$ 2D Fun. Ele. $\rightarrow$ 3D Fun. Ele." projection strategy using lightweight detectors. 
Instead of traversing all frames, the detection and segmentation process only needs to be applied to the selected top-$k$ frames with respect to each object node. 
This yields two main advantages:
\begin{enumerate}
    \item \textbf{High computational efficiency:}  As shown in our newly added runtime comparison \Cref{table:times}, our method processes scenes significantly faster.
    \item \textbf{Structural robustness:} By segmenting functional elements within the 2D bounding boxes of projected 3D objects and projecting back to the 3D object point cloud, the parent-child edges between objects and functional elements are naturally established, eliminating the complex and error-prone graph-edge association step required by other methods.
\end{enumerate}

To validate our design choices, we have added a comprehensive ablation study in \Cref{sec:eval_graph}. 
The new results quantitatively demonstrate that aggregating features from optimal views significantly improves both part detection recall and open-vocabulary retrieval accuracy.

\subsection{Regarding Tracking Comparison}
The primary reason we compared against hand-tracking and point-tracking methods is that functional elements on articulated objects are often heavily occluded by human hands during manipulation, making direct vision-only functional element tracking exceptionally fragile. 

However, we strongly agree with the reviewer's broader point: our framework is inherently \textit{agnostic} to the underlying tracking method. Any tracking algorithm can be plugged in to supply the trajectories. 
We utilized the hardware-assisted gripper specifically to provide the highest possible accuracy for direct, reliable robotic execution. 
% We have added a discussion in the text clarifying the "plug-and-play" nature of our framework regarding tracking modules.

\subsection{Regarding Adding Baseline FunGraph}
We deeply appreciate this suggestion. 
As shown in \Cref{sec:eval_graph}, we have removed Lost\&Found and replaced it with the more appropriate FunGraph baseline.

\subsection{Regarding Evaluation Dataset Selection}
We have revised our manuscript in \Cref{sec:eval_graph} to explicitly frame real-world environments as our primary evaluation focus, as they best validate our human-interaction pipeline. 
For simulation, we choose Behavior-1K over SceneFun3D because its environments are densely populated with articulated objects, perfectly aligning with our manipulation focus. 
Conversely, SceneFun3D targets static segmentation across broader, non-articulable affordances (e.g., light switches), making it incompatible with our full dynamic pipeline. 
To validate the robustness of our static initialization module on a standardized benchmark, we also evaluate it on SceneFun3D. 
As shown in \Cref{table:scenefun3d}, on the 4 affordance types specifically relevant to articulation objects, our method achieves comparable average performance to FunGraph.
